C-RAN with Hybrid RF/FSO Fronthaul Links: Joint Optimization of RF Time Allocation and Fronthaul Compression

This paper considers the uplink of a cloud radio access network (C-RAN) comprised of several multi-antenna remote radio units (RUs) which compress the signals that they receive from multiple mobile users (MUs) and forward them to a CU via wireless fronthaul links. To enable reliable high rate fronthaul links, we employ a hybrid radio frequency (RF)/free space optical (FSO) system for fronthauling. To strike a balance between complexity and performance, we consider three different quantization schemes at the RUs, namely per-antenna vector quantization (AVQ), per-RU vector quantization (RVQ), and distributed source coding (DSC), and two different receivers at the CU, namely the linear minimum mean square error receiver and the optimal successive interference cancellation receiver. For this network architecture, we investigate the joint optimization of the quantization noise covariance matrices at the RUs and the RF time allocation to the multiple-access and fronthaul links for rate region maximization. To this end, we formulate a unified weighted sum rate maximization problem valid for each possible pair of the considered quantization and detection schemes. To handle the non-convexity of the unified problem, we transform it into a bi-convex problem which facilitates the derivation of an efficient suboptimal solution using alternating convex optimization and golden section search. Our simulation results show that for each pair of the considered quantization and detection schemes, C-RAN with hybrid RF/FSO fronthauling can achieve a considerable sum rate gain compared to conventional systems employing pure FSO fronthauling, especially under unfavorable atmospheric conditions. Moreover, employing a more sophisticated quantization scheme can significantly improve the system performance under adverse atmospheric conditions.

==> Fig/Complexity_D/Complexity.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA Scenario 3\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA Scenario 2\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Scenario 1\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB Relative complexity}%
\psfrag{024}[tc][tc]{\matlabtextB Total number of antennas at the RUs $x$}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextC $\mathcal{O}(x)$}%
\psfrag{021}[cl][cl]{\matlabtextC $\mathcal{O}(x^2)$}%
\psfrag{022}[cl][cl]{\matlabtextC $\mathcal{O}(x^3)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $4$}%
\psfrag{001}[ct][ct]{\matlabtextD $6$}%
\psfrag{002}[ct][ct]{\matlabtextD $8$}%
\psfrag{003}[ct][ct]{\matlabtextD $10$}%
\psfrag{004}[ct][ct]{\matlabtextD $12$}%
\psfrag{005}[ct][ct]{\matlabtextD $14$}%
\psfrag{006}[ct][ct]{\matlabtextD $16$}%
\psfrag{007}[ct][ct]{\matlabtextD $18$}%
\psfrag{008}[ct][ct]{\matlabtextD $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextD $10^{0}$}%
\psfrag{010}[rc][rc]{\matlabtextD $10^{1}$}%
\psfrag{011}[rc][rc]{\matlabtextD $10^{2}$}%
\psfrag{012}[rc][rc]{\matlabtextD $10^{3}$}%
\psfrag{013}[rc][rc]{\matlabtextD $10^{4}$}%
%
%% </ytick>

==> Fig/Complexity_Q/Complexity.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA Scenario 3\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Scenario 2\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA Scenario 1\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB Relative complexity}%
\psfrag{028}[tc][tc]{\matlabtextB Total number of antennas at the RUs $x$}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextC $\mathcal{O}(x)$}%
\psfrag{024}[cl][cl]{\matlabtextC $\mathcal{O}(x2^{\sqrt{x}})$}%
\psfrag{025}[cl][cl]{\matlabtextC $\mathcal{O}(x\sqrt{2^{x}})$}%
\psfrag{026}[cl][cl]{\matlabtextC $\mathcal{O}(x2^{x})$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $4$}%
\psfrag{001}[ct][ct]{\matlabtextD $6$}%
\psfrag{002}[ct][ct]{\matlabtextD $8$}%
\psfrag{003}[ct][ct]{\matlabtextD $10$}%
\psfrag{004}[ct][ct]{\matlabtextD $12$}%
\psfrag{005}[ct][ct]{\matlabtextD $14$}%
\psfrag{006}[ct][ct]{\matlabtextD $16$}%
\psfrag{007}[ct][ct]{\matlabtextD $18$}%
\psfrag{008}[ct][ct]{\matlabtextD $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextD $10^{0}$}%
\psfrag{010}[rc][rc]{\matlabtextD $10^{1}$}%
\psfrag{011}[rc][rc]{\matlabtextD $10^{2}$}%
\psfrag{012}[rc][rc]{\matlabtextD $10^{3}$}%
\psfrag{013}[rc][rc]{\matlabtextD $10^{4}$}%
\psfrag{014}[rc][rc]{\matlabtextD $10^{5}$}%
\psfrag{015}[rc][rc]{\matlabtextD $10^{6}$}%
\psfrag{016}[rc][rc]{\matlabtextD $10^{7}$}%
%
%% </ytick>

==> Fig/RateRegion_k50/RateRegion.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA MMSE Receiver\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA SIC Receiver\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA V-MAC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB $R_2$ (Mbps)}%
\psfrag{021}[tc][tc]{\matlabtextB $R_1$ (Mbps)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $150$}%
\psfrag{004}[ct][ct]{\matlabtextC $200$}%
\psfrag{005}[ct][ct]{\matlabtextC $250$}%
\psfrag{006}[ct][ct]{\matlabtextC $300$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $50$}%
\psfrag{009}[rc][rc]{\matlabtextC $100$}%
\psfrag{010}[rc][rc]{\matlabtextC $150$}%
\psfrag{011}[rc][rc]{\matlabtextC $200$}%
\psfrag{012}[rc][rc]{\matlabtextC $250$}%
\psfrag{013}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Fig/RateRegion_k80/RateRegion.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA MMSE Receiver\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA SIC Receiver\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA V-MAC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB $R_2$ (Mbps)}%
\psfrag{021}[tc][tc]{\matlabtextB $R_1$ (Mbps)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $150$}%
\psfrag{004}[ct][ct]{\matlabtextC $200$}%
\psfrag{005}[ct][ct]{\matlabtextC $250$}%
\psfrag{006}[ct][ct]{\matlabtextC $300$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $50$}%
\psfrag{009}[rc][rc]{\matlabtextC $100$}%
\psfrag{010}[rc][rc]{\matlabtextC $150$}%
\psfrag{011}[rc][rc]{\matlabtextC $200$}%
\psfrag{012}[rc][rc]{\matlabtextC $250$}%
\psfrag{013}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Fig/SumRate_P_N/SumRate_P.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA MMSE Receiver\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA SIC Receiver\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA $N=8$\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA $N=6$\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA $N=4$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextB $110$ Mbps gain}%
\psfrag{025}[cl][cl]{\matlabtextB $130$ Mbps gain}%
\psfrag{026}[cl][cl]{\matlabtextB $190$ Mbps gain}%
\psfrag{027}[bc][bc]{\matlabtextB Average Sum Rate (Mbps)}%
\psfrag{028}[tc][tc]{\matlabtextB $P$ (dBm)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $25$}%
\psfrag{006}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $200$}%
\psfrag{009}[rc][rc]{\matlabtextC $300$}%
\psfrag{010}[rc][rc]{\matlabtextC $400$}%
\psfrag{011}[rc][rc]{\matlabtextC $500$}%
\psfrag{012}[rc][rc]{\matlabtextC $600$}%
\psfrag{013}[rc][rc]{\matlabtextC $700$}%
\psfrag{014}[rc][rc]{\matlabtextC $800$}%
\psfrag{015}[rc][rc]{\matlabtextC $900$}%
\psfrag{016}[rc][rc]{\matlabtextC $1000$}%
\psfrag{017}[rc][rc]{\matlabtextC $1100$}%
\psfrag{018}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Fig/SumRate_alpha/SumRate_alpha.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA MMSE Receiver\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA SIC Receiver\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{025}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{026}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[cl][cl]{\matlabtextB $500$ Mbps gain}%
\psfrag{028}[bc][bc]{\matlabtextB Sum Rate (Mbps)}%
\psfrag{029}[tc][tc]{\matlabtextB $\alpha_0$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.7$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{009}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
\psfrag{013}[rc][rc]{\matlabtextC $200$}%
\psfrag{014}[rc][rc]{\matlabtextC $300$}%
\psfrag{015}[rc][rc]{\matlabtextC $400$}%
\psfrag{016}[rc][rc]{\matlabtextC $500$}%
\psfrag{017}[rc][rc]{\matlabtextC $600$}%
\psfrag{018}[rc][rc]{\matlabtextC $700$}%
\psfrag{019}[rc][rc]{\matlabtextC $800$}%
\psfrag{020}[rc][rc]{\matlabtextC $900$}%
\psfrag{021}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Fig/SumRate_alpha_k50/SumRate_alpha.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA MMSE Receiver\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA SIC Receiver\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA AVQ\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA RVQ\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[cl][cl]{\matlabtextB $130$ Mbps gain}%
\psfrag{026}[cl][cl]{\matlabtextB $300$ Mbps gain}%
\psfrag{027}[bc][bc]{\matlabtextB Sum Rate (Mbps)}%
\psfrag{028}[tc][tc]{\matlabtextB $\alpha_0$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.7$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{009}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $200$}%
\psfrag{013}[rc][rc]{\matlabtextC $400$}%
\psfrag{014}[rc][rc]{\matlabtextC $600$}%
\psfrag{015}[rc][rc]{\matlabtextC $800$}%
\psfrag{016}[rc][rc]{\matlabtextC $1000$}%
\psfrag{017}[rc][rc]{\matlabtextC $1200$}%
\psfrag{018}[rc][rc]{\matlabtextC $1400$}%
\psfrag{019}[rc][rc]{\matlabtextC $1600$}%
%
%% </ytick>

==> Fig/SumRate_kappa/SumRate_kappa.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA MMSE Detector\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA MMSE-DFE Detector\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA SQ\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA VQ\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA DSC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Sumrate (Mbps)}%
\psfrag{022}[tc][tc]{\matlabtextB $\kappa\times 10^{3}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $60$}%
\psfrag{004}[ct][ct]{\matlabtextC $80$}%
\psfrag{005}[ct][ct]{\matlabtextC $100$}%
\psfrag{006}[ct][ct]{\matlabtextC $120$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $150$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
\psfrag{010}[rc][rc]{\matlabtextC $250$}%
\psfrag{011}[rc][rc]{\matlabtextC $300$}%
\psfrag{012}[rc][rc]{\matlabtextC $350$}%
\psfrag{013}[rc][rc]{\matlabtextC $400$}%
\psfrag{014}[rc][rc]{\matlabtextC $450$}%
\psfrag{015}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>
